Exploring Author Gender in Book Rating and Recommendation

Collaborative filtering algorithms find useful patterns in rating and consumption data and exploit these patterns to guide users to good items. Many of the patterns in rating datasets reflect important real-world differences between the various users and items in the data; other patterns may be irrelevant or possibly undesirable for social or ethical reasons, particularly if they reflect undesired discrimination, such as discrimination in publishing or purchasing against authors who are women or ethnic minorities. In this work, we examine the response of collaborative filtering recommender algorithms to the distribution of their input data with respect to a dimension of social concern, namely content creator gender. Using publicly-available book ratings data, we measure the distribution of the genders of the authors of books in user rating profiles and recommendation lists produced from this data. We find that common collaborative filtering algorithms differ in the gender distribution of their recommendation lists, and in the relationship of that output distribution to user profile distribution.

==> 00-preamble.tex <==
\section*{Preamble}

Our paper addresses the question ``how do collaborative filtering algorithms interact with issues of gender representation in book authorship?''.
It presents extensive data sets, experimental methodologies, and research results confirming that collaborative filtering algorithms propagate users' tendencies with regard to author gender into resulting recommendation lists, which was not a given in light of previous results that collaborative filters do not propagate all input patterns.

We spend considerable space expositing a methodology for answering questions of this form, in significantly more detail than can be achieved in a conference paper.  It is our belief that this extended justification, along with a thorough accounting of our results, merits journal publication.

This paper addresses the question of how a socially-relevant content creator characteristic --- author gender --- is latently handled by user modeling and recommendation techniques that do not have any explicit notion of it.  This is a valuable prerequisite for further exploration of fairness and social effects in user modeling and its resulting applications.

The main limitations of our approach are (1) the current dependency on binary gender constructs and (2) the computational complexity of the statistical methods.

Besides our own previous conference paper, the calibration work of \citet{steck_calibrated_2018} and recommender-independence analysis of \citet{Kamishima2018-ri} are the two most related papers we know.  Both of these papers are concerned with ensuring certain kinds of fairness, and develop sophisticated algorithms for doing so; in contrast, we are concerned with understanding what existing algorithms do.

\subsection*{Relationship to Conference Paper}
This is extended version of our RecSys 2018 paper \citep{bag-recsys18}.  We have made significant extensions to the contextualization, exposition, rigor, reproducibility, and generalizability of our findings:

\begin{itemize}
    \item An extended introduction situates this work in the broader space of fair recommendation and provides a strengthened normative justification for this particular fairness construct.
    \item We present substantially more detail about our data collection and integration, as well as our experimental design, describing and justifying the decisions made throughout the pipeline in more detail than a conference paper could afford.  This expansion will make this version of the paper a more useful starting point for others seeking to engage in similar research.
    \item We expand our experiments to include an additional data set from GoodReads, improving the generalizability of the results.
    \item We changed to the Python version of LensKit and replaced the FunkSVD and Poisson factorization algorithms with ALS and BPR.  The result is that we are now using a matrix factorization technique that is appropriate to implicit feedback (the FunkSVD implementation from the Java version of LensKit was not), and we include results on a representative learning-to-rank technique.
    \item We reran all experiments with a documented and reproducible hyperparameter tuning strategy.  In addition to improving the experiment's reproducibility, running with better-performing algorithms fixes a key limitation of the original paper in that it was unclear how results would hold on better-performing algorithm configurations.
\end{itemize}

==> ext-abstract.tex <==
% Content for the 3-page extended abstract

\section{Introduction}

The evaluation of recommender systems has historically focused on the accuracy of recommendations.  
When it is concerned with other characteristics, such as diversity, novelty, and user satisfaction, it often continues to focus on traditionally-understood information needs.  But this paradigm, while irreplaceable in creating products that deliver immediate value, does not tell the whole story of a recommender system's interaction with its users, content creators, and other stakeholders.


In this paper, we report observational results from our investigation into how recommender systems interact with author gender in book data and associated consumption and rating patterns.
The goal of this paper is to characterize the distribution of author genders in existing book data sets and the response of common collaborative filtering algorithms to that distribution.
We address four research questions:

\begin{description}
\item[RQ1] How are author genders distributed in book catalog data?
\item[RQ2] How are author genders distributed in users' book reading histories?
\item[RQ3] What is the distribution of author genders in the recommendations users receive from common collaborative filtering algorithms? This measures the \emph{overall} behavior of the recommender algorithm(s) with respect to author gender.
\item[RQ4] How do individual users’ gender distributions propagate into the recommendations that they receive? This measures the \emph{personalized} gender behavior of the algorithms.
\item[RQ5] How much accuracy must be sacrificed to force recommendation lists to have particular gender balances? 
\end{description}

In addition, we consider the \emph{temporal evolution} of RQ2, looking for change in book rating patterns over time, particularly before and after GoodReads added algorithmic recommendation to its platform.

\section{Methods}

We study these questions by training common collaborative filtering algorithms on publicly-available book data.
We use the BookCrossing, Amazon, and GoodReads data sets, generate recommendations with algorithms supplied by LensKit for Python, and analyze user profiles, recommendation lists, and their relationships with a hierarchical Bayesian model.
We operationalize gender balance as the proportion of books by authors with known gender identities that are written by women; there are limitations to this approach discussed in the full paper, but it enables us to make forward progress on this important question.

\section{Results}

Overall, we find that (RQ1) books in our database are significantly more likely to be written by men than by women, but representation is more balanced among rated books; (RQ2) users are diffuse in their rating tendencies, with an overall trend favoring male authors but this trend is less strong than the baseline distribution; (RQ3) different CF techniques produce recommendations with quite different distributions; and (RQ4) most algorithms reflected some of each user's profile tendency into their recommendations, particularly in implicit feedback settings. RQ5 and temporal results are in progress as of abstract time.

\section{Relationship to Previous Paper}

This paper is an expansion of our RecSys 2018 paper \citep{bag-recsys18}.
with new and updated material substantially increasing scope and reliability:

\begin{enumerate}
    \item \textbf{Expanded and refined data sets}, adding rating data from GoodReads \citep{monotonic} and using the Library of Congress Authority File to obtain higher-quality author data connected to books and ratings through linking identifiers.http://localhost:8888/?token=7a90901d43d7b7f51244b7441747c8f54d6da236aaacfcbf
    \item \textbf{Infrastructure update} to use LensKit for Python \citep{lkpy} to drive the experiments and
    re-optimize algorithm hyperparameters using scikit-optimize, enabling easier reproducibility with lower computing resource requirements and higher algorithm accuracy.
    \item \textbf{Expanded algorithm set}, in particular adding exemplars of algorithm families not represented in the original paper (BPR-MF for Learning-to-Rank and WRMF for implicit-feedback-oriented matrix factorization).
    \item \textbf{Expanded analysis}, assessing the (in)stability of gender representation in user ratings over time, examining the effect of GoodRead's introduction of a recommender system to its platform, and validating analysis tecnniques with a neutral control bias.
    \item \textbf{Bias adjustment}, evaluating the impact of greedy re-ranking to alter or maintain specific gender distributions in book recommendation lists.
\end{enumerate}

